Tokenization Preference for Human and Machine Learning Model: An Annotation Study

Is preferred tokenization for humans also preferred for machine-learning (ML) models? This study examines the relations between preferred tokenization for humans (appropriateness and readability) and one for ML models (performance on an NLP task). The question texts of the Japanese commonsense question-answering dataset are tokenized with six different tokenizers, and the performances of human annotators and ML models were compared. Furthermore, we analyze relations among performance of answers by human and ML model, the appropriateness of tokenization for human, and response time to questions by human. This study provides a quantitative investigation result that shows that preferred tokenizations for humans and ML models are not necessarily always the same. The result also implies that existing methods using language models for tokenization could be a good compromise both for human and ML models.

==> tables/annotation_result_30sec.tex <==

\begin{table*}[ht]
\centering
\small
\begin{tabular}{l|r|rrr|rrr|rrr}
\hline
         & \multicolumn{1}{r|}{Readability} & \multicolumn{3}{r|}{Accuracy}                         & \multicolumn{3}{r|}{Averaged Answer Time}                  & \multicolumn{3}{r}{Averaged Token Length}                   \\
         & Train                       & Train          & Valid          & Total          & Train         & Valid         & Total         &  
 Train          & Valid          & Total         \\ \hline
 MeCab    & \textbf{68.23}             & \textbf{93.90} & \textbf{97.50} & \textbf{94.30} & 5.44          & 5.09          & 5.40          & 9.70            & 7.04         & 9.61          \\
Unigram  & 16.38                      & 93.85          & 97.40           & 94.25          & 5.37          & \u{ 5.02}    & 5.33          & 7.66           & 5.78         & 7.59          \\
BPE      & 5.97                       & \textbf{93.90} & 97.32          & 94.28          & 5.44          & 5.06          & 5.40          & 7.40            & \u{ 5.54}   & 7.34          \\
MaxMatch & 4.12                       & 93.69          & \textbf{97.50} & 94.11          & 5.42          & 5.17          & 5.39          & \u{ 7.35}     & 5.55         & \u{ 7.29}    \\
OpTok    & 4.09                       & 93.69          & \u{ 97.05}    & 94.06          & \u{ 5.35}    & 5.04          & \u{ 5.31}    & 7.98           & 5.88         & 7.91          \\
Random   & \u{ 1.21}                 & \u{ 93.23}    & 97.23          & \u{ 93.67}    & \textbf{6.06} & \textbf{5.98} & \textbf{6.05} & \textbf{10.03} & \textbf{7.40} & \textbf{9.94} \\ \hline
\end{tabular}
\caption{
    foo.
    %各トークン分割手法で問題文を区切って提示した際の，読みやすさ1位の割合（\%，学習データの3,302件）と正解率（\%），平均回答時間（単位は秒，正答・回答時間が30秒以内のサンプルのみを集計），各サンプルの問題文の平均トークン数．
    %列内の\textbf{最大値を太字}，\underline{最小値を下線}でハイライトした．
    \label{tbl:annotation_result}
}
\end{table*}

==> tables/cl_performance.tex <==
\begin{table}[t]
\centering
\begin{tabular}{lrr}
\hline
         & Bag-of-Words & BiLSTM \\\hline
MeCab    & 42.48       & 44.06  \\
Unigram  & 43.97       & \textbf{44.80} \\
BPE      & \textbf{44.15}       & 44.53 \\
MaxMatch & 43.61       & 44.74  \\
OpTok    & 43.37       & 44.30 \\
Random   & \underline{41.94}       & \underline{42.39}  \\
\hline
\end{tabular}
\caption{
    foo.
    %JCommonsenseQAでの正解率（検証データ）．
    %列内の\textbf{最大値を太字}，\underline{最小値を下線}でハイライトした．
    \label{tbl:cl_performance}
}
\end{table}

==> tables/column_result.tex <==
\begin{table*}[ht]
\centering
\begin{tabular}{lrrrrrr}
\hline
                 & MeCab & Unigram  & BPE   & MaxMatch & OpTok  & Random        \\ \hline
\textit{Accuracy of Human (\%)} &   &        &        &         &             &               \\
Train            & 94.71  & 94.76     & 94.77   & 94.87   & \b{94.93}    & \u{94.48}      \\
Valid            & 96.51  & \b{97.32}     & 96.87   & 96.96   & 96.78    & \u{96.34}           \\
Total            & 94.91  & 95.05     & 95.01   & 95.10   & \b{95.14}    & \u{94.69}  \\ \hline
\textit{Response Time (sec.)}     &                &                &                &                &             &               \\
Train            & 4.02  & 3.99     & 4.00   & \u{3.94}   & 3.97    & \b{4.09}    \\
Valid            & 2.89  & 2.91     & 2.91   & \b{2.98}   & \u{2.82}    & 2.96          \\
Total            & 3.89  & 3.86     & 3.88   & \u{3.83}   & 3.84    & \b{3.96}   \\ \hline
\end{tabular}
\caption{
    The performance of machiineML learning models and annotation results for the JCommonsenseQA dataset with six tokenization methods.
    The highest and lowest values in each raw are highlighted with bold and underline, respectively.
    %各トークン分割手法で問題文を区切って提示した際の，読みやすさ1位の割合（\%，学習データの3,302件）と正解率（\%），平均回答時間（単位は秒，正答・回答時間が30秒以内のサンプルのみを集計），各サンプルの問題文の平均トークン数．
    \label{tbl:column_result}
}
\end{table*}


==> tables/shuffled_result.tex <==
\begin{table*}[ht]
\centering
\begin{tabular}{lrrrrrr}
\hline
                               & MeCab      & Unigram & BPE        & MaxMatch   & OpTok  & Random         \\ \hline
\textit{Size of Vocabulary}    &            &         &            &            &        &                \\
Vocab of Tokenizer             & -          & 64,000  & 64,000     & 64,000     & 64,000 & -              \\
Vocab Used in Train            & 8,692      & 11,227  & 11,597     & 12,152     & 10,758 & 17,528      \\ 
Vocab Used in Valid            & 2,418      & 3,101   & 3,290      &  3,367     & 2,966  & 3,952          \\   
Vocab Used in Total            & 9,267      & 11,921  & 12,292     & 12,890     & 11,440 & 19,077         \\ \hline
\textit{Tokenization Length} &              &         &            &            &        &                \\
Train                          & 10.20      & 8.02    & 7.77       & \u{7.71}       & 8.39   & \b{10.56}         \\
Valid                          & 10.32      & 8.11    & 7.93       & \u{7.86}       & 8.49   & \b{10.68}       \\
Total                          & 10.21      & 8.03    & 7.79       & \u{7.73}  & 8.40   & \b{10.58}  \\ \hline
\textit{Entropy}               &            &         &            &            &        &                \\
Train                          & \u{8.27}   & 9.68    & 10.18      & 10.23      & 9.35   & \b{10.40}          \\
Valid                          & 8.91       & 9.08    & 9.52       & 9.56       & \u{8.80}   &\b{9.75}          \\
Total                          & \u{8.29} & 9.71    & 10.20      & 10.25      & 9.38   & \b{10.43} \\ \hline
\hline
\textit{Accuracy of Machine}    &                &                &       &          &                &               \\
Valid (Bag-of-Words)            & 39.92          & \b{41.91} & 40.75 & 41.41    & 41.29          & \u{39.29}   \\
Valid (BiLSTM)                  & 42.12          & 43.61          & 42.95 & 42.90    & \b{44.15} & \u{40.57}   \\ \hline
\textit{Appropriateness}        &                &                &       &          &                &               \\
Train                           & \u{1.86}     & 2.65           & 3.14  & 2.94     & 2.56           & \b{5.60} \\
Valid                           & \u{1.87}     & 2.67           & 3.13  & 2.98     & 2.50           & \b{5.61} \\
Total                           & \u{1.86}     & 2.65           & 3.14  & 2.95     & 2.55           & \b{5.61} \\ \hline
Accuracy of Human               &                &                &       &          &                &               \\
Train                           & \b{94.22} & 94.03          & 94.17 & 94.03    & 93.88          & \u{93.58}   \\
Valid                           & 95.08          & \b{95.97} & 95.17 & 94.72    & 95.53          & \u{94.45}   \\
Total                           & \b{94.30} & 94.25          & 94.28 & 94.11    & 94.06          & \u{93.67}   \\ \hline
\textit{Averaged Response Time} &                &                &       &          &                &               \\
Train                           & 5.44           & 5.37           & 5.44  & 5.42     & \u{5.35}     & \b{5.06} \\
Valid                           & 5.09           & \u{5.03}     & 5.07  & 5.17     & 5.05           & \b{5.98} \\
Total                           & 5.40           & 5.33           & 5.40  & 5.39     & \u{5.31}     & \b{6.05} \\ \hline
\end{tabular}
\caption{
    Tokenization information and experimental results on the newly created training/validation splits.
}
\label{tbl:result_shuffle}
\end{table*}

% annotation以外の情報をまとめる？
% perplexityとか、30秒以上かかったやつとか
% tokenizationの差は、table2とマージしてしまうと見やすいかも

==> tables/vocabSize.tex <==
\begin{table}[t]
\centering
\begin{tabular}{lrr}
\hline
          & |V|    & V in QA \\ \hline
MeCab     & -      & 9,267  \\
Unigram   & 64,000 & 11,921  \\
BPE       & 64,000 & 12,292  \\
MaxMatch & 64,000 & 12,890  \\
OpTok     & 64,000 & 11,440  \\
Random    & -      & 19,077  \\ \hline
\end{tabular}
\caption{
    %トークナイゼーション手法ごとの語彙の規模
    foo.
    \label{tbl:vocabSize}
}
\end{table}
